Comparing two cohomological obstructions for contextuality, and a generalised construction of quantum advantage with shallow circuits

We present two results on the subject of quantum contextuality and cohomology, and non-locality and quantum advantage with shallow circuits. Abramsky et al. showed that a range of examples of quantum contextuality is detected by a cohomological invariant based on \v{C}ech cohomology. However, the approach does not give a complete cohomological characterisation of contextuality. A different cohomological approach to contextuality was introduced by Okay et al. Their approach exploits the algebraic structure of the Pauli operators and their qudit generalisations known as Weyl operators. We give an abstract account of this structure, then generalise their approach to any example of contextuality with this structure. We prove at this general level that the approach does not give a more complete characterisation of contextuality than the \v{C}ech cohomology approach. Bravyi, Gosset, and K\"{o}nig (BGK) gave the first unconditional proof that a restricted class of quantum circuits is more powerful than its classical analogue. The result, for the class of circuits of bounded depth and fan-in (shallow circuits), exploits a particular family of examples of contextuality. BGK's quantum circuit and computational problem are derived from a family of non-local games related to the well-known GHZ non-local game. We present a generalised version of their construction. A systematic way of taking examples of contextuality and producing unconditional quantum advantage results with shallow circuits.

==> acknowledgements.tex <==
\begin{acknowledgements}
    Thank you Samson, Rui, Shane, Gio, Nadish,
    Sparebank1 Ringerike Hadeland, and Aker Scholarship, \dots
\end{acknowledgements}

==> shallow-circuits.tex <==
\chapter{Quantum Advantage with Shallow Circuits}
The subject of this chapter is the increased computational power
of shallow quantum circuits, as shown by Bravyi, Gosset, and K\"{o}nig,
and the role of contextuality in enabling this advantage.
We restrict attention to multipartite contextuality, which is also
known as \emph{non-locality} when measurement sites are spatially separated.
We show that the role of a particular example of contextuality
in BGK's result is that it can simulate it in a uniform way.
We then present two generalisations of this result.

\paragraph{Structure of chapter} In Section \ref{section:shallow-circuits}
we first introduce shallow circuits. In Section \ref{section:generating-circuit}
we make the idea of generating
an empirical model with a circuit precise.
In Section \ref{section:lightcones} we consider the problem
of detecting that an empirical model that is generated by a shallow quantum
circuit is not generated by a shallow classical circuit.
To do this we use the idea of \emph{restrictions}, looking at the behaviour
of circuits when all but a small number of inputs are fixed.
We explain that this approach can detect that an empirical model
cannot be generated by a shallow classical circuit,
but it cannot detect a difference between shallow quantum and shallow classical circuits.

In Section \ref{section:bgk-result} we present BGK's result.
In Section \ref{section:graph-states} we introduce the trick for creating
entanglement between qubits that are far away.
We then use this to define the precise circuit and relational problem
considered by BGK.
After this we restate the result in terms of a simulation
that works like a refined version of the
restrictions we considered in Section \ref{section:lightcones}.

In the remainder of the chapter we present two generalisations of the result
presented in this resource theoretic way.
In Section \ref{section:distributing-weyl} we present a construction
that allows us to define a distributed version of a Weyl realisable empirical model.
In Section \ref{section-single-round-result} we use this construction
to lift a Weyl realisable empirical model to a family of models
and prove quantum advantage.
In Section \ref{section:distributing-all-measurements} we explain the restriction
to Weyl measurements can be removed if we instead consider
two-round empirical models.
In Section \ref{section:two-round-result} we present a version
of the result for a more general type of circuit, called \emph{interactive circuits}.

\section{Shallow circuits} \label{section:shallow-circuits}
A circuit is a directed acyclic graph (DAG)
with three types of nodes: inputs, outputs, and gates.
By evaluating the gates according to the graph structure
the circuit defines a function, or more generally a probabilistic function,
from the space of input values to the space of output values.
The \emph{depth} of a circuit is the length of the longest path
from an input to an output. The \emph{fan-in} of a gate is the number of inputs,
or equivalently the input degree of the graph node corresponding to the gate.
The \emph{maximal fan-in} of a circuit is the maximal fan-in over all of the gates.
\begin{definition}
    A \emph{shallow circuit} is a family
    of circuits $F = \{F_n\}_{n \in \nats}$
    for which there exists $K,D \in \nats$ such
    that $F_n$ has depth at most $D$ and maximal fan-in
    at most $K$ for all $n \in \nats$.
\end{definition}

We are concerned with circuits of a particular form
that we call \emph{generating circuits}.
\subsection{Generating empirical models with circuits} \label{section:generating-circuit}
Informally, a generating circuit is a classical or quantum circuit
whose behaviour is an empirical model.

\begin{definition}
Let $S = (I, \{X_i\}_{i \in I}, \{Y_{i,x}\}_{i \in I, x \in X_i})$
be a multipartite scenario. A \emph{generating circuit}
is a deterministic classical circuit or a quantum circuit having for each $i \in I$:
\begin{itemize}
    \item A classical input $\text{in}_i$ of type $X_i$.
    \item A classical output $\text{out}_i$, such that if the input value
    to $\text{in}_i$ is $x \in X_i$, then the output value of $\text{out}_i$
    has type $Y_{i,x}$.
    \end{itemize}
Additionally a \emph{quantum generating circuit} can use any number of qudits
prepared in the computational basis state,
and a \emph{classical generating circuit} can use any number of additional inputs
initialised according to a random seed.
\end{definition}

Note that any classical probabilistic circuit is equivalent to a deterministic circuit
with an additional random seed. Let $F=C,Q$ be a classical or quantum generating circuit.
The \emph{empirical model generated by $F$} is defined for each joint input $x = \{x_i\}_{i \in I}$
by setting input $\text{in}_i$ to $x_i$, evaluating the circuit,
reading of the values of outputs $\{\text{out}_i\}_{i \in I}$
and discarding the additional outputs.
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics{quantum-generator.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics{classical-generator.pdf}
    \end{subfigure}
\end{figure}

\textbf{Comment about notation} To simplify notation we will write $F$, instead of $e$,
for the empirical model generated by $F$, if it is clear from the context what is meant.

\subsection{Empirical models generated by shallow circuits} \label{section:lightcones}
Non-contextual empirical models are convex combinations
of deterministic outcome assignments, such that
the outcome at each measurement site is a function of only the measurement
setting at the same measurement site.
\begin{equation}
    e = x \mapsto \sum_{\lambda} p_\lambda \cdot \big(f_{\lambda,i}(x_i)\big)_{i \in I}
\end{equation}
Empirical models generated by classical circuits of low depth
and fan-in can be given a similar description.

\begin{definition}
    Let $F$ be a circuit with inputs $\{\text{in}_i\}_{i \in I}$ and outputs $\{\text{out}_j\}_{j \in J}$.
    The \emph{forward lightcone} $\lcf{F}(i) \subset J$ is the set of all outputs
    that are reachable from input $i \in I$,
    and the \emph{backward lightcone} $\lcb{F}(j) \subset I$ is the set of all inputs
    that can reach output $j \in J$
    \begin{align}
        i \in \lcb{F}(j) \iff 
        j \in \lcf{F}(i) \iff
            \text{there is a path in $F$ from $\text{in}_i$ to $\text{out}_j$}
    \end{align}
\end{definition}

Suppose that $e$ is generated by a classical generating circuit $C$ of depth
$D$ and maximal fan-in $K$. We can then write $e$ as a convex combination
\begin{equation}
    e = x \mapsto \sum_z p_z \cdot \big( f_{z,i}(\res{x}{\lcb{C}(i)}) \big)_{i \in I}
\end{equation}
where $f_{z,i}(\res{x}{\lcb{C}(i)})$ is the unique value determined by evaluating
$C$. Note that
\begin{equation}
    \supp{\lcb{C}(i)} \leq K^D
\end{equation}

\paragraph{Restricting classical circuits}
A restriction $r = (I', x_0)$ consists of a set of measurement sites $I' \subset I$
and a joint measurement $x_0$ for the remaining measurements sites.
Write $\res{e}{r}, \res{f}{r}$ for the restricted empirical model,
and restricted function given by fixing the value of the remaining inputs according to $x_0$.

Applying the restriction $r$ to the empirical model $e$ generated by $C$ gives
\begin{equation}
    \res{e}{r} = x \mapsto \sum_{z} p_z \cdot \big(\res{f_{z,i}}{r}(\res{x}{I' \cap \lcb{C}(i)})\big)_{i \in I}
\end{equation}
Hence, if $I' \cap \lcb{C}(i) \subset \{i\}$ for all $i \in I'$ then $\res{e}{r}$ is non-contextual.

Suppose now that $K^D$ and $\supp{I'}$ are both small compared to $\supp{I}$,
and that $r$ is chosen randomly such that $I'$ is uniformly distributed.
It can then be shown using a union bound that the probability
that there exists $i \neq i' \in I'$ such that $i \in \lcb{C}(i')$ is small.
Hence also the probability that $\res{e}{r}$ is contextual is small.
This shows that if a family of empirical models is generated by
a shallow quantum circuit, then they cannot behave contextually
in a distributed way.

\paragraph{Restricting quantum circuits}
That $e$ is generated by a quantum circuit of depth $D$ and maximal fan-in $K$.
If the restricted model $\res{e}{r}$ is contextual
then there must be $i \neq i'$ such that $\lcb{Q}(i) \cap \lcb{Q}(i') \neq \emptyset$,
because otherwise the model would factorise.
However, we can use a simple combinatorial argument to show
that the probability of this happening when
$r$ is chosen uniformly at random is $\alpha (K^D)^2 \supp{I}^{-1}$.
However, we can similarly show using the union bound that this probability
is small. Hence $\res{e'}{r}$ is also non-contextual
with high probability.

To be able to distinguish between shallow quantum and classical circuits
BGK uses a more refined notion of restriction
which we describe as a simulation.



Hence we can only detect a constant difference. Not sufficiently powerful to differentiate
between shallow quantum and shallow classical circuits.

\section{Bravyi, Gosset, and K\"{o}nig's result} \label{section:bgk-result}

\begin{definition}
    Let $G = (V, E, r)$ be a rooted graph, $I$ a finite set, and $d \geq 2$.
    $\text{Scenario}(G, I, d)$ is the multipartite scenario
    with measurement sites $I \times V$
    and the following measurement settings.
    At each measurement site $(i,r)$:
    \begin{itemize}
            \item A measurement $p$, for each $p \in \mathbb{Z}_d^2$,
            with outcomes $\mathbb{Z}_d$.
            \item A measurement $w$, for each \emph{neighbour} $w \in N_G(r)$, with outcomes $\mathbb{Z}_d^2$.
    \end{itemize}
    At each measurement site $(i,v)$, where $v \neq r$:
    \begin{itemize}
            \item A measurement $(w,p)$, for each $p \in \mathbb{Z}_d^2$
            and $w \in N_G(v)$, with outcomes $\mathbb{Z}_d$.
            \item A measurement $(w,w')$, for each pair of 
                \emph{neighbours} $w \neq w' \in N_G(v)$, with outcomes $\mathbb{Z}_d^2$.
    \end{itemize}
\end{definition}

\begin{definition}
    Let $G = (V,E,r)$ be a rooted graph, $d \geq 2$, $I$
    a finite set, and $\ket{\psi}$ an $I$-qudit state.
    $\text{Realisation}(G,I,d,\psi)$ is the quantum
    realisation for $\text{Scenario}(G,I,d)$ with state
    \begin{equation}
        \ket{\psi, G} 
            := \ket{\psi} \otimes \bigotimes_{i \in I, e \in E} \ket{\phi}_{i,e}
    \end{equation}
    and the following interpretation of the measurement
    settings.
    At each measurement site $(i,r)$:
    \begin{itemize}
        \item $p$ is the Pauli measurement $W(p)$ applied to qudit 
            $i$.
        \item $w$ is a Bell basis measurement applied to qudits
        $i$ and $(i,r,w)$.
    \end{itemize}
    At each measurement site $(i,v)$, where $v \neq r$:
    \begin{itemize}
        \item $(w,p)$ is the Pauli measurement $W(p)$ applied to 
            qudit $(i,v,w)$.
        \item $(w,w')$ is a Bell basis measurement applied to qudits
        $(i,v,w)$ and $(i,v,w')$.
    \end{itemize}
\end{definition}

\begin{definition}
    Let $G = (V,E,r)$ be a rooted graph, $I$ a finite set, $d \geq 2$,
    and $\pmb{v} = \{(v_{i1}, \dots, v_{il_i})\}_{i \in I}$ a choice
    of rooted paths.
    $\text{Simulation}(G,I,d,\pmb{v})$ is the following deterministic
    simulation from $\text{Scenario}(G,I,d)$ to 
    $(I, \{\mathbb{Z}_d^2\}, \{\mathbb{Z}_d\})$.
    Given a joint measurement $\{p_i \in \mathbb{Z}_d^2\}_{i \in I}$
    for $(I, \{\mathbb{Z}_d^2\}, \{\mathbb{Z}_d\})$:
    \begin{itemize}
        \item If $l_i=1$ then measure $(i,r)$ with $p_i$ otherwise measure $(i,r)$ with $v_{i,2}$.
        \item Measure $(i,v_{ij})$ with $(v_{i(j-1)}, v_{i(j+1)})$, for each $i=2,\dots,l_i-1$.
        \item Measure $(i, v_{il_i})$ with $(p_i, v_{i(l_i-1)})$.
    \end{itemize}
    Given a joint outcome $\{y_{i,v}\}_{i \in I, v \in V}$
    return $y_{i,v} + [y_i, p_i]$ where
    $y_i := \bigoplus_{i=1}^{l_i} y_{i,v}$.
\end{definition}

In the previous section we explained that shallow classical circuits
cannot behave contextually in a uniform way. However, that
a quantum circuit that behaves distributedely contextual needs to create entanglement
between qubits that are far away.
To do this BGK relies upon an earlier result
by Barrett et al.\ \cite{barrett_modeling_2007} about modelling
Pauli measurements on graph states using nearest neighbour communication.

\subsection{Creating long-distance entanglement with local operations}

\begin{definition}
    Let $G = (V,E)$ be a graph. The \emph{graph state} $\ket{G}$
    is the $V$-qubit state defined by
    \begin{equation} \label{eq:graph-state-def}
        \ket{G} := \big( \prod_{\{v,w\} \in E} CZ_{v,w} \big) H^{\otimes V} \ket{0}^{\otimes V}
    \end{equation}
    where $CZ_{v,w}$ is the controlled $Z$ gate applied between qubit $v$ and $w$,
    and $H$ is the Hadamard gate.
\end{definition}

Barrett et al.\ considers a cyclic graph state with three nodes $A,B,C$.
This state can be prepared quantum mechanically by applying controlled $Z$
gates between nearest neighbours.
Barrett et al.'s observation is that any classical model
for this system requires the communication of measurement settings
between nodes that are far away with respect to the graph structure.

\subsection{The 2D-GHZ game: Playing the GHZ game on a grid} \label{section:graph-states}
BGK strengthens this result by considering Pauli measurements on the graph states of
$n \times n$ grids. For each embedding of a cycle into the grid
Barrett et al.'s result emposes a communication requirement on any classical model
for the grid. We can fix one node and vary the other nodes in many different ways.
For each of these variations some of the nodes that are far away needs to communicate
to $B$. Overall there is therefore a large number of nodes that need to communicate to $B$.

To recast this result in the language of circuits observe that
because the $CZ$ gates commute they can be arranged into $4$ layers
of parallel gates. The model is therefore generated by a shallow quantum circuit.

\begin{definition}
    Let $Q_n$ be the quantum circuit that prepares the graph state $\ket{\text{Grid}(n,n)}$
    and applies a controlled Pauli measurement on each qubit, for each $n \in \nats$.
\end{definition}
\begin{definition}
    Let $Q_n$ be the quantum generating circuit
    of type $([n^2], \{\mathbb{Z}_{2}^2\}, \{\mathbb{Z}_2\})$
    that prepares the graph state $\ket{\text{Grid}(n,n)}$
    of the $n \times n$ grid,
    and measures each qubit with a classically
    controlled Pauli measurement.
\end{definition}

If $C_n$ is any classical circuit then there is only $K^D$ outputs that can receive
information from any input, however, by the previous argument
any classical model requires communication from many inputs. Hence $C_n$ is not equivalent
to $Q_n$. We now explain that there is a concrete computational problem witnessing this.

Barrett et al.\ considers the following version of the GHZ game played by the nodes
of the cycle.

To understand this observe that the $X$ measurements creates a GHZ state
shared between $A,B,C$, up to a random Pauli phase at each qubit.
The phases are random, hence it doesn't violate no-signalling. However,
with knowledge of the phases we can implement a winning strategy for the GHZ-game.
This phase commutes through a Pauli measurement up to a relabelling of the measurement outcomes.
The ``correction'' is the required relabelling. Hence it solves the game perfectly
because the GHZ strategy solves the GHZ game perfectly.
In the classical case note that a classical model requires communication.
However, if none of the outcomes depend on ... then it doesn't communicate
between any of the players.

By choosing the embedding randomly in a ``sufficiently uniform'' way
it follows that the result problem, called the 2D-GHZ problem
is not solved efficiently by any classical shallow circuit.

\begin{definition}
    The \emph{2D-GHZ game} $\Phi_{\text{GHZ}}(n)$ is defined by
\end{definition}

\begin{customthm}{(BGK)}
    The shallow circuit $\{Q\text{-2D-GHZ}(n)\}_{n \in \nats}$
    solves the 2D-GHZ game perfectly for all $n \in \nats$.
    However, no classical shallow circuit solves it with high accuracy.
   There exists a shallow family of quantum generating circuits $\{Q_n\}_{n \in \nats}$
   and cooperative games $\{\Phi_n\}_{n \in \nats}$ such
   that $Q_n$ solves $\Phi_n$ perfectly for all $n \in \nats$.
   However, if  $\{C_n\}_{n \in \nats}$
   is a classical shallow generating circuit
   then there exists $\epsilon_n \in O(1/n)$
   such that 
   \begin{align}
       p_S(Q_n, \Phi_n) &= 1\\
       p_S(C_n, \Phi_n) &\leq 3/4 + \epsilon_n
   \end{align}
\end{customthm}

\begin{figure}
    \centering
    \begin{subfigure}{0.2\textwidth}
        \includegraphics[width=1\textwidth]{barrett-state.pdf} 
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \includegraphics[width=1\textwidth]{bgk-state.pdf} 
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \includegraphics[scale=1.1]{prepare-measure-circuit.pdf}
        \caption{}\label{fig:quantum-circuit}
    \end{subfigure}
    \caption{Caption}
\end{figure}

Note that the transformation $U_n$ can be implemented by a shallow
quantum circuit because the $CZ$ gates in Equation (\ref{eq:graph-state-def}) can be arranged into four 
layers of parallel gates. To see this note that a decomposition
of the gates into $k$ layers of parallel gates is equivalent to an edge colouring of the grid
using $k$ colours.

Let $q = (v_A, v_B, v_C, \bar{u}_A, \bar{u}_C, \bar{u}_C)$
denote a tuple consisting of nodes $v_A,v_B,v_C \in \text{Grid}(n,n)$
and paths $\bar{u}_A$ from $v_B$ to $v_C$, $\bar{u}_B$ from $v_A$ to $v_C$, 
and $\bar{u}_C$ from $v_B$ to $v_A$.
For each $q$ and $x_A,x_B,x_C \in \mathbb{Z}_2$
we define a joint measurement$x(q,x_A,x_B,x_C) \in (\mathbb{Z}_2^2)^{n^2}$
\begin{equation}
    x(q,x_A,x_B,x_C) := \begin{cases}
        v_A \mapsto (1, x_A), &\\
        v_B \mapsto (1, x_B), &\\
        v_C \mapsto (1, x_C), &\\
        v \mapsto (1,0), &\text{if $v \in \supp{\bar{u}_A} \cup \supp{\bar{u}_B} \cup \supp{\bar{u}_C}$}\\
        v \mapsto (0,1), &\text{otherwise}
    \end{cases}
\end{equation}
and an accepting condition $A_n(q,x_A,x_B,x_C) \subset (\mathbb{Z}_2)^{n^2}$ by
\begin{equation}
    y \in A_n(q,x_A,x_B,x_C) \iff
    x_A \lor x_B \lor x_C =
    \bigoplus_{P=A,B,C} (y_P + x_P \cdot y_{P\text{-Odd}} + y_{P\text{-Even}})
\end{equation}
where
\begin{align}
    y_{P\text{-Odd}} := \bigoplus_{\text{odd } i} y(\bar{u}_P(i)),
    \quad \quad
    y_{P\text{-Even}} := \bigoplus_{\text{even } i} y(\bar{u}_P(i))
\end{align}

Let $x(q)$ be the input that 

The cooperative game is given by a relation $A_n \subset \mathbb{Z}_4^{n^2} \times \mathbb{Z}_2^{n^2}$,
and a probability distribution $d_n \in \dist(\mathbb{Z}_4^{n^2})$.
\begin{definition}
    Let 
    $y \in (\mathbb{Z}_2)^{n^2}$ satisfies the constrain if and only if
\end{definition}

The probability distribution $d_n$ is defined such that $A,B,C$ are uniformly
chosen, $(x_A,x_B,x_C)$ such that $x_A \lor x_B \lor x_C = 0$
with uniform probability, and the paths have even minimal length.

\subsection{Proving quantum advantage for the 2D-GHZ game}
The proof of BGK's result can be understood in terms of a simulation.
The intuition is similar to the restriction thing we presented earlier.
However, the simulations we use alllows for more flexibility
so that the quantum circuit can produce entanglement.

For each $q$ we can define a deterministic simulation
let $s_n(q):([n]^2, \{\mathbb{Z}_2^2\}, \{\mathbb{Z}_2\}) \to (\{A,B,C\}, \{\mathbb{Z}_2\}, \{\mathbb{Z}_2\})$
such that the induced maps are
\begin{align}
    f(q)&::(x_A,x_B,x_C) \mapsto x(q,x_A,x_B,x_C)\\
    g(q)&::(x_A,x_B,x_C,y) \mapsto \big(y_P + x_P \cdot y_{P\text{-Odd}} + y_{P\text{-Even}}\big)_{P=A,B,C}
\end{align}
let $s_n:([n]^2, \{\mathbb{Z}_2^2\}, \{\mathbb{Z}_2\}) \to (\{A,B,C\}, \{\mathbb{Z}_2\}, \{\mathbb{Z}_2\})$
be the probabilitistic simulation given by choosing $q$ randomly according to the distibution
$u_n$ used in BGK's result
\begin{equation}
    s_n := \sum_{q} u_n(q) \cdot s_n(q)
\end{equation}
The 2D-GHZ game is then the pullback of the GHZ game
\begin{equation}
    \text{2D-GHZ}(n) = {s_n}^*(\text{GHZ-Game})
\end{equation}

By the defining property of the pullback it is then equivalent to show that
\begin{align}
    p_S({s_n}_*(Q_n), \Phi_{\text{GHZ}}) &= 1\\
    p_S({s_n}_*(C_n), \Phi_{\text{GHZ}}) &\leq 3/4 + \epsilon_n
\end{align}
Now, recall that $e_\text{GHZ}$ succeeds with certainty at the GHZ game,
and that we have a resource inequality 
$p_S(e, \Phi) \leq \gamma + \cf{e}$,
for any non-local game $(\Phi, \gamma)$ and empirical model $e$.
It is therefore sufficient to show that
\begin{align}
    {s_n}_*(Q_n) &= e_\text{GHZ}\\
    \cf{{s_n}_*(C_n)} &\leq \epsilon_n
\end{align}

Now note that the essence of what we explained in the previous section
is that this is the case. For some more detail
on the classical side we can write
the behaviour of a classical circuit as a convex combination

we therefore get the following expression for the pushforward.
\begin{equation}
    s_n(q)_*(e) = x \mapsto \sum_{z} p_z \cdot \big( f_{z,i}(\res{x}{\lcb{C}(i)}) \big)_{i \in I}
\end{equation}
Now note that because of the resticted dependencies
it works essentially as the restictions.
If there are no ... and .. such that ..., then the pushforward
deterministic model is non-contextual.
Hence the contextual fraction is bounded by the probability
that this is the case.

\begin{align}
    g(x_A,x_B,x_C, \big( f_{z,i}(\res{x(q, x_A,x_B,x_C)}{\lcb{C}(v)}) \big)_{v \in [n]^2})_P
\end{align}

The expressions for the actual maps in the simulation
\begin{align}
    f_P(v_P,\bar{u}_P)(x) &:=
    \begin{cases}
        v_P \mapsto (1, x),  &\text{if $w = v$}\\
        v \mapsto (1,0), &\text{otherwise}
    \end{cases}\\
    g_P(q, v_P, y) &:= y_P + x_P \cdot y_{P\text{-Odd}} + y_{P\text{-Even}}
\end{align}

In this argument observe that the role of the GHZ game
can be echanged with any non-local game for which
$e_\text{GHZ}$ demonstrates quantum advantage.
If $(\Phi, \gamma)$ is any non-local game,
and $\Phi_n := {s_n}^*(\Phi)$, then
\begin{align}
    p_S(e_n, \Phi_n) &= p_S(e_{\text{GHZ}}, \Phi)\\
    p_S(e_n', \Phi_n) &\leq \gamma + \epsilon_n
\end{align}
In this sense the simulations $s_n$ are a more fundamental witness of quantum
advantage.

\section{Generalised quantum advantage result with shallow circuits} \label{section:distributing-weyl}
The key to BGK's result is that the cluster states can be prepared by
a shallow quantum circuit. Yet by measuring with local measurements
along paths we can create an entangled GHZ state, up to a random phase,
between qubits that are far away.
This trick allows us to relate the behaviour of the cluster state
models to the GHZ model in a distributed way.
Furthermore, this simulation allows us to pull back any witness of contextuality
to a witness of quantum advantage with shallow circuits.

The goal of this section is to define a distributed version of any model uses only Weyl operator
measurements for any $d$ and on any state, not necessarily stabiliser.

In their result the structure is the grid.
This works because the GHZ state is special.
Our strategy is different.
We use a state consisting of any
multi-qudit entangled state and an additional number of entangled two-qudit
states. Using a trick based on teleportation
we show that the qudits of the multi-qudit state
can be indepenently distribued around the state.
In the next section we use this to construct quantum advantage
results.

\begin{figure}
    \centering
    \hfill
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[scale=1]{3x3x3-grid.pdf}
        \caption{}\label{fig:3x3x3-grid}
   \end{subfigure}
    \hfill
    \vrule
    \hfill
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[scale=1]{t22.pdf}
        \caption{}\label{fig:t22}
    \end{subfigure}
    \hfill{}
    \caption{
        Examples of rooted graphs. The circle denotes the root node.
        (a) A 3-dimensional hypergrid. (b) A binary tree. 
    }
\end{figure}

\subsection{Distributing entanglement with teleportation}
Let $\ket{\phi}$ denote the two-qudit \emph{maximally entangled state}
and write $\mathcal{B}$ for the \emph{Bell basis},
the two-qudit basis generated by applying the Weyl operators
to one of the qudits of $\ket{\phi}$.
\begin{align}
    \ket{\phi} &:= \frac{1}{\sqrt{d}} \sum_{j} \ket{j} \ket{j}\\
    \mathcal{B} &:= \{\ket{\phi_p} := (I \otimes W(p))\ket{\phi} \}_{p \in \mathbb{Z}_d^2}
\end{align}

In the standard teleportation protocol for qudits a single-qudit state $\ket{\psi}$
and one of the qudits of $\ket{\phi}$ are measured in the Bell basis,
giving an outcome $p \in \mathbb{Z}_2$. The post-measurement state
of the final qudit is then, up to the Weyl operator phase $W(p)$,
the original state $\ket{\psi}$. By performing a correction $W(p)^\dagger$
we can hence retrieve the original state. Expressed diagrammatically:
\begin{equation} \label{eq:bell-identity}
  \vcenter{\hbox{\includegraphics{bell-identity.pdf}}}
\end{equation}

\paragraph{Parallel Bell basis measurements}
If we want to teleport a state more than one step we can simply apply the standard protocol
$n$ times. However, because of the composition law of Weyl operators
we can instead perform the $n$ Bell basis measurements in parallel and
perform a single correction at the end.
Using graphical notation
\begin{equation}
    \vcenter{\hbox{\includegraphics{bell-identity-iterated.pdf}}}
\end{equation}

\paragraph{Using a graph as a template}
\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{resource-state-step-1.pdf}
        \caption{}
        \label{fig:measurement-setting}
    \end{subfigure}
    \hfill
    \vrule
    \hfill
    \begin{subfigure}{0.48\textwidth}
    \centering
        \includegraphics[width=1\textwidth]{resource-state-step-2.pdf}
        \caption{}
        \label{fig:step-two}
    \end{subfigure}
    \caption{(a) On input $x(\bar{v}, p)$ the circuit $Q(\psi,G)$ uses Bell basis measurements
    to entangle each qudit of $\psi$
    with a qudit that is far away in the circuit and measures this qudit in the Weyl basis.
    (b) The effect of the Bell basis measurements is to teleport $\psi$
    up to a random phase.
    }
    \label{fig:teleportation}
\end{figure}

\begin{definition}
    A \emph{rooted graph} $G = (V,E,r)$ is an undirected and connected graph with
    a distinguished node $r$ called the root.
    A \emph{path} in $G$ is a non-repetitive list of 
    nodes $r = v_1, v_2, \dots, v_l$
    starting with the root such that consecutive pairs $v_i,v_{i+1}$ are adjacent.
\end{definition}

In this section we will fix an arbitrary $I$-qudit state $\ket{\psi}$
and a rooted graph $G = (V,E,r)$. $G$ will serve as a template for distributing
$\ket{\psi}$ with teleportation. 

We now define the quantum state, denoted by $\ket{\psi,G}$ that the protocol acts upon.
$\ket{\psi,G}$ is a state of a multi-qudit register
with qudits labelled by
\begin{equation}
    I \cup \{(i,v,w) \in I \times V^2 \mid \{v,w\} \in E\}
\end{equation}

\begin{definition}
    Let $\ket{\psi,G}$ be the product of $\ket{\psi}$
    with a maximally entangled state $\ket{\phi}_{(i, v,w), (i, w,v)}$
    for each $i \in I, \{v,w\} \in E$.
    \begin{equation}
        \ket{\psi,G} := \ket{\psi} \otimes \bigotimes_{i \in I, \{v,w\} \in E} \ket{\phi}_{(i,v,w), (i,w,v)}
    \end{equation}
\end{definition}

Note that $\ket{\psi,G}$ is a product state and does not have any further structure
on its own. However, by grouping the qudits together it inherits
a graph structure from $G$.
For each $(i,v) \in I \times V$ let $N_G(i,v)$ be the following subset of qudits
\begin{equation}
    N_G(i,v) := \begin{cases}
        \{i\} \cup \{(i,v,w) \mid \{v,w\} \in E\}, &\text{if $v = r$}\\
        \{(i,v,w) \mid \{v,w\} \in E\}, &\text{otherwise}
    \end{cases}
\end{equation}
Observe that with respect to these subsets the \emph{root cells}
$\{N_G(i,r)\}_{i \in I}$ each hold one qudit of $\ket{\psi}$,
and each pair of adjacent cells $N(i,w), N(i,v)$, such that $\{v,w\} \in E$
shares a maximally entangled pair of qudits.
However, by applying local Bell basis measurements
at each cell we can teleport each qudit
to an arbitary chosen cell using a path.

\begin{lemma} \label{lemma:parallel-teleportation}
    Let $\pmb{v} = \big( (v_{i1}, \dots, v_{il_i}) \in \text{Paths}(G) \big)_{i \in I}$ be a 
    family of paths.
    Suppose that for each $i \in I$ 
    qudits $i$ and $(i, v_{i2}, v_{i1})$
    as well as qudits $(i, v_{ij}, v_{i(j-1)})$ and $(i, v_{ij}, v_{i(j+1))}$
    for all $j=1,\dots,l_i-1$
    are measured in the Bell basis with
    with outcomes $p_{i1}, \dots, p_{i(l_i-1)} \in \mathbb{Z}_d$.
    
    The post measurement state of qudits
    $\{(i, v_{il_i}, v_{i(l_i-1)})\}_{i \in I}$,
    is then $\big[ \bigotimes_{i \in I} W(p_i) \big] \ket{\psi}$,
    where
    \begin{equation}
        p_i := p_{i1} + \dots + p_{i(l_i-1)}
    \end{equation}
\end{lemma}
\begin{proof}
    Consider first the case that $\ket{\psi}$ is a single-qudit state.
    By iteratively applying identity (\ref{eq:bell-identity})
    to each measurement along each path
    we have that the post measurement state
    us
    \begin{equation}
        \big[ \bigotimes_{i \in I} W(p_{i(l_i-1)}) \dots W(p_{i1}) \big] \ket{\psi}
    \end{equation}
    Using the composition law of Weyl operators
    we can collect the phases into a single phase
    that is equivalent up to a global unobservable phase
    \begin{equation}
        \big[ \bigotimes_{i \in I} W(p_{i(l_i-1)}) \dots W(p_{i1}) \big] \ket{\psi}
        \approx
        \big[ \bigotimes_{i \in I} W(p_{i(l_i-1)} + \dots + p_{i1}) \big] \ket{\psi}
    \end{equation}
    as required.
\end{proof}


\subsection{Distributed Weyl measurement models}
\begin{definition}
    Let $I$ be a set, $d \geq 2$, and $\ket{\psi}$
    an $I$-qudit state.
    The \emph{Weyl measurement model} $e_\psi:(I, \{\mathbb{Z}_d^2\}, \{\mathbb{Z}_d\})$
    is the empirical model given interpreting measurement
    setting $(i,p)$ as the Weyl measurement $W(p)$ applied to
    qudit $i$ of $\ket{\psi}$.
\end{definition}

Let $e_\psi:(I, \{\mathbb{Z}_d^2\}, \{\mathbb{Z}_d\})$ be a Weyl measurement model
and $G = (V,E,r)$ a rooted graph.
For any choice of paths $\pmb{v}$ and Weyl measurement setting $\pmb{p}$
suppose that we simultaneously apply the teleportation protocol
along $\pmb{v}$ and perform the Weyl measurements at the final qudits.
By Lemma the state being measured 

Let $\ket{\psi}$ be an $I$-qudit state and $W(p_i)$ a Weyl measurement
for each qudit $i \in I$. Suppose that we perform the sequence
of Bell basis measurements along a choice of paths for each qudit
on the state $\ket{\psi,G}$ for some rooted graph $G$,
and simultaneously apply $W(p_i)$ to the final qudit.
By Lemma \ref{lemma:parallel-teleportation} the state
of the measured qudits is then $\big[ \bigotimes_{i \in I} W(p_i') \big] \ket{\psi}$.
However, by Lemma \label{lemma:permutation-lemma}
the effect of measuring this state with the Weyl measurements
$\big[ \bigotimes_{i \in I} W(p_i) \big]$, is up to a permutation of the outcomes
equivalent to measuring $\ket{\psi}$.
Returning the outcome $i \mapsto q_i + [p_i, p_i']$ is then equivelent
to measuring $\ket{\psi}$.

\begin{align}
    \Bigg[ \bigotimes_{i \in I} \bra{p_i, q_i} \Bigg] \Bigg[ \bigotimes_{i \in I} W(p_i') \Bigg]
    \ket{\psi}
    \approx
    \Bigg[ \bigotimes_{i \in I} \bra{p_i, q_i + [p_i, p_i']} \Bigg] \ket{\psi}
\end{align}

We can therfore use $\ket{\psi,G}$ to simulate Weyl measurements on $\ket{\psi}$
using local measurements. We now introduce a measurement scenario
$T(I,d,G)$ that encodes the operations used here classically,
and a simulation $s(I,d,G)$ that expresses the operations of this distributed protocol.

\begin{lemma} \label{lemma:permutation-lemma}
    Let $\ket{p,q}$ be an $\omega^q$-eigenvector of the Weyl operator
    $W(p)$. For any $p,p' \in \mathbb{Z}_d^2$ and $q \in \mathbb{Z}_d$
    \begin{equation}
        W(p')\ket{p,q} \approx \ket{p, q + [p,p']}
    \end{equation}
\end{lemma}
\begin{proof}
    We have
    \begin{align}
        W(p)W(p')\ket{p,q} &= \omega^{[p,p']}W(p')W(p)\ket{p,q}\\
        &= \omega^{[p,p']}W(p')\omega^q\ket{p,q}
    \end{align}
\end{proof}

To implement $e_{\psi,W}$ in a distributed way
we can therefore randomly select a path, teleport perform the correct for the outcome
afterwards.
We encode the information required to this classically
using the following multipartite scenario.

\begin{definition} 
    Let $T(I,d,G) := (I \times V, \{X_i\}_{i \in I}, \{Y_{i,x}\}_{i \in I, x \in X_i})$
    be the multipartite scenario
    with measurement settings $X_{i,v}$
    for each $(i,v) \in I \times V$
    \begin{equation}
        X_{i,v} := \begin{cases}
            p \mid w, &\text{if $v = r$}\\
            (w,p) \mid (w,w') \mid \bullet, &\text{otherwise}
        \end{cases}
    \end{equation}
    where $p \in \mathbb{Z}_d^2$, $\{v,w\} \neq \{v,w'\} \in E$,
    and the outcomes $Y_{i,v,x}$
    for each $(i,v) \in I \times V$ and $x \in X_i$
    \begin{equation}
        Y_{i,r,x} := \begin{cases}
            \mathbb{Z}_d, &\text{if $x = p$}\\
            \mathbb{Z}_d^2, &\text{if $x = w$}
        \end{cases},
        \quad
        Y_{i,v,x} := \begin{cases}
            \mathbb{Z}_d, &\text{if $x = (w,p)$}\\
            \mathbb{Z}_d^2, &\text{if $x = (w,w')$}
        \end{cases}
    \end{equation}
    for each $i \in I, r \neq v \in V$.
\end{definition}

The empirical model we consider is given by interpreting
$p \in X_{i,r}$ as the Weyl measurement $W(p)$
applied to qudit $i$, $w \in X_{i,r}$
as a Bell basis measurement applied to qudit $i$
and qudit $(i, r, w)$,
$(p,w) \in X_{i,v}$ as the Weyl measurement
$W(p)$ applied to qudit $(i,v,w)$,
and $(w,w') \in X_{i,v}$
as the Bell basis measurement on qudits $(i,v,w), (i,v,w')$.

\begin{definition}
    Let $e_{\psi,W}(G)$ be the empirical model
    of type $T(I,d,G)$ given by measuring $\ket{\psi,G}$ with measurements
    \begin{equation}
        \tau(I,d,G)(i,r) := \begin{cases}
            w \mapsto \mathcal{B}_{i, (i, r, w)}, &\\
            p \mapsto W(p)_i, &\\
            \bullet \mapsto \text{id}_{N_G(i,r)}
        \end{cases},
        \quad
        \tau(I,d,G)(i,v) := \begin{cases}
            (w,w') \mapsto \mathcal{B}_{(i,v,w), (i, w, v)}, &\\
            (w,p) \mapsto W(p)_w, &\\
            \bullet \mapsto \text{id}_{N_G(i,v)}
        \end{cases}
    \end{equation}
\end{definition}
        
\paragraph{Simulation}
For any path $(v_1, \dots, v_l) \in \text{Paths}(G)$
write $f_i(\pmb{v})(p)$
for the joint measurement for measurement sites
$\{i\} \times \supp{\pmb{v}}$
\begin{equation}
    f_i(\pmb{v})(p) := (i,v) \mapsto \begin{cases}
        v_2, &\text{if $v = v_1$}\\
        (v_{j-1}, v_{j+1}), &\text{if $v=v_2, \dots, v_{l-1}$}\\
        (v_{l-1}, p), &\text{if $v = v_l$}
   \end{cases} 
\end{equation}
In other words, when acting on the empirical model
the effect is to apply Bell basis measurements along the path and $W(p)$
at the final qudit
\begin{figure}[h]
      \centering
        \includegraphics{1d-1r-teleport-final.pdf}
\end{figure}

Let $g_i(\pmb{v})$ be the outcome with the correction
factor from the outcomes along the path
\begin{equation}
    g_i(\pmb{v}) := (p,y) \mapsto y_{i,v_l} + [p, y_{i,v_1} + \dots + y_{i,v_{l-1}}]
\end{equation}

\begin{definition}
    For each choice of paths $\pmb{v} = \big( \pmb{v}_i \in \text{Paths}(G) \big)_{i \in I}$
    let $s(I,d,G,\pmb{v}):T(I,d,G) \to S(I,d)$
    be the deterministic simulation
    \begin{equation}
        s(I,d,G,\pmb{v}) :=
            ( \big(\{i\} \times \supp{\pmb{v}_i} \big)_{i \in I}, \big( f_i(\pmb{v}_i) \big)_{i \in I},
                \big(g_i(\pmb{v}_i) \big)_{i \in I}
            )
    \end{equation}
\end{definition}

\begin{definition}
    For any path distribution $u \in \dist(\text{Paths}(G))$
    let $s(I,d,G,u):T(I,d,G) \to S(I,d)$ be the probabilistic simulation
    \begin{equation}
        s(I,d,G,u) := \sum_{\pmb{v}} \prod_{i \in I} u(\pmb{v}_i) \cdot s(I,d,G,\pmb{v})
    \end{equation}
\end{definition}

\begin{lemma} \label{lemma:simulation-one-round}
    For any path distribution $u$
    the simulation $s(I,d,G,u)$ simulates $e_{\psi,W}$
    using $e_{\psi,W}(G)$ as a resource.
\end{lemma}
\begin{proof}
    The proof follows from Lemma \ref{lemma:parallel-teleportation}
    and Lemma \ref{lemma:permutation-lemma}.
\end{proof}

\subsection{Generating distributed Weyl measurement models with shallow circuits} \label{section-single-round-result}
\begin{definition}
    Let $G = (V,E,r)$ be a rooted graph.
    The \emph{radius} of $G$
    is the maximal distance from the root to any node,
    and the \emph{maximal degree} is the maximal number of neighbours to any single node.
    \begin{align*}
            \text{rad}(G) &:= \text{max}_{v \in V}\ \text{min}
                \{l \mid (v_1 = r, \dots, v_l = v) \in \text{Paths}(G)\}
                \\
            \text{deg}(G) &:= \text{max}_{v \in V} \supp{\{w \mid \{v,w\} \in E\}}
    \end{align*}
\end{definition}

The state $\ket{\psi,G}$ can be prepared by a depth one circuit
consisting of a single gate $U_\psi$ of fan-in $\supp{I}$
and a number of fan-in two gates $U_e$.
Because the measurements are performed on each cell
and each cell contains at most 

\begin{figure}
    \centering
        \includegraphics[width=0.45\textwidth]{circuit-definition.pdf}
        \caption{} \label{fig:circuit-definition}
\end{figure}

\begin{definition} \label{def:quantum-circuit-one}
    Let $Q(I,d,\psi,G)$ be the following quantum generating circuit
    of type $T(I,d,G)$.
    $Q(I,d,\psi,G)$ consists of a unitary layer of gates
    $U_\psi \otimes \bigotimes_{e \in E} U_e$
    followed by a classically controlled measurement gate
    $M_{i,v}$ that uses
    input $(i,v)$ to apply measurement $\tau(I,d,G)(i, x_{i,v})$.
\end{definition}
    
    To prepare the state $\ket{\psi,G}$ the circuit
    uses a single fan-in $\supp{I}$ gate $U_\psi$,
    and a fan-in two gate $U_{i,e}$ for each $i \in I, e \in E$,
    applied in parallel.
    The state $\ket{\psi,G}$ is measured
    using a classically controlled measurement gate
    $M(i,v)$ acting on qudits $N_G(i,v)$
    and the outcome is returned.
    By definition it is easily seen that the circuit
    has depth two and maximal fan-in $\text{max}(\supp{I}, \Delta(G)+2)$.
    A generating circuit for $e$ is shown in Figure \ref{fig:circuit-definition}.

Let $e$ be the empirical model with quantum realisation
$(\ket{\psi,G}, \tau(I,d,G))$.
$e$ is generated by a quantum circuit of depth two and maximal fan-in 
$\text{max}(\supp{I}, \Delta(G) + 2)$.

\begin{customthm}{I}
    Let $e_{\psi,W}:(I, \{\mathbb{Z}_d^2\}, \{\mathbb{Z}_d\})$
    be a Weyl measurement model, $\{G_n\}_{n \in \nats}$ rooted graphs of bounded degree,
    and $\{u_n \in \dist(\text{Paths}(G_n))\}_{n \in \nats}$
    such that when $v_1, \dots, v_l$ is chosen randomly from $u_n$
    \begin{enumerate}
        \item the endpoint $v_l$ is uniformly distributed,
        \item the length of $v_1, \dots, v_l$ is at most the radius of $G$.
    \end{enumerate}
    
    $\{Q_n := Q(I,d,\psi,G_n)\}_{n \in \nats}$ is shallow and $Q_n$ simulates 
    $e_{\psi,W}$ through $s_n := s(I,d,G_n,u_n)$
    for each $n \in \nats$.
    However, the empirical models simulated
    by any shallow classical generating circuit $\{C_n\}_{n \in \nats}$
    through $\{s_n\}_{n \in \nats}$ have bounded contextual fraction:
    \begin{align}
        {s_n}_*(Q_n) &= e_{\psi,W}\\
        \cf{{s_n}_*(C_n)} &\in O(\supp{G_n}^{-1}\text{rad}(G_n))
    \end{align} 
\end{customthm}
\begin{proof}
    Quantum circuits are often represented on a standard form
    consisting of a number of unitary multi-qubit gates
    followed by a computational basis measurement.
    It should be clear that the quantum circuits
    we define are equivalent to quantum circuits
    on the standard form
    with an at most $O(1)$ increase in depth and maximal fan-in.
    (2.) follows from Lemma \ref{lemma:simulation-one-round}.
    The lemmas used for (1.) and (3.) is proved in the remainder of the section.
    In Lemma \ref{lemma:quantum-circuit-lemma} we show
    that $e_n$ is generated by a quantum circuit
    of depth two and maximal fan-in $\text{max}(\supp{I}, \Delta(G_n) + 2)$.
    In Lemma \ref{lemma:classical-bound} we show that 
    $\cf{{s(I,d,G, u)}_*(e')} \leq \supp{I}^2 K^D \supp{G}^{-1} \text{rad}(G)$.
\end{proof}

Some relevant examples of rooted graphs
are hypergrid graphs, and tree graphs.
\begin{example}
    The \emph{hypergrid graph} $[n]^k$, where $n,k \in \nats$,
    generalise the line and the two-dimensional square grid to higher dimension.
    The set of nodes is $\{(a_1, \dots, a_k) \mid a_1, \dots, a_k \in \{1,\dots,n\}\}$,
    root $(1,\dots, 1)$,
    and $(a_1, \dots, a_k), (b_1,\dots, b_k)$ are adjacent
    if $\supp{a_j - b_j} = 1$ for some $j$
    and $a_{j'} = b_{j'}$ for all $j' \neq j$.
\end{example}
\begin{example}
    $T_{k,n}$ is the \emph{$k$-ary tree of depth $n$}.
    The set of nodes is $\{(i,j) \mid i \in \{1,\dots,n\}, j \in \{1, \dots, k^{i-1}\}\}$,
    root $(1,1)$,
    and $(i,j), (i',j')$ are adjacent if $i' = i + 1$ and $k(j-1) < j' \leq kj$.
\end{example}


\begin{example}
    For any fixed $k \in \nats$ consider Theorem I with
    $G_n := [n]^k$.
    Then $\{Q_n\}_{n \in \nats}$ is shallow.
    However, $\cf{{s_n}_*(C_n)} \in O(k^{n-1})$
    for any classical shallow circuit $\{C_n\}_{n \in \nats}$.
\end{example}

\begin{example}
    For any fixed $k \in \nats$
    consider Theorem I with $G_n = T_{n,k}$.
    Then $\{Q_n\}_{n \in \nats}$ is shallow (but has exponential size).
    However, $\cf{{s_n}_*(C_n)} \in O(n^{k-1})$
    for any classical shallow circuit $\{C_n\}_{n \in \nats}$.
\end{example}

\subsection{Classical bound}
The proof of the classical bound (Lemma \ref{lemma:classical-bound})
relies upon two lemmas.
In Lemma \ref{lemma:lightcones-lemma} we give a condition
ensuring that the pushforward ${s(I,d,G,\pmb{v})}_*(e)$ is non-contextual
in terms of the lightcones of a classical circuit $C$
generating $e$ and the choice of paths $\pmb{v}$.
Lemma \ref{lemma:bgks-lemma} which is adapted from \cite{bravyi_quantum_2018}
allows us to bound the probability of this condition happening
when $\pmb{v}$ is chosen in a sufficiently uniform way.

\begin{lemma} \label{lemma:lightcones-lemma}
    Let $C$ be a classical generating circuit of type $T(I,d,G)$
    and $\pmb{v} = \{(v_{i1}, \dots, v_{il_i}) \in \text{Paths}(G)\}_{i \in I}$ a choice of paths.
    If there are no $i \neq i' \in I$
    with $\{v_{i1}, \dots, v_{il_i}\} \cap \lcf{C}(i', v_{i'l_{i'}}) \neq \emptyset$
    then the empirical model 
    ${s(I,d,G, \pmb{v})}_*(C)$
    simulated by $C$ through $s(I,d,G, \pmb{v})$
    is non-contextual.
\end{lemma}
\begin{proof}
    The empirical model generated by $C$ can be expressed
    as a convex combination of a family of functions
    $\{h_z\}_z$
    \begin{align}
        x \mapsto \sum_z p_z \cdot h_z(x)
    \end{align}
    such that the value of $h_z(x)$ at $(i,v)$
    is only a function of the value of $x$ at $\lcb{C}(i,v)$
    \begin{equation}
        h_z::x \mapsto \big( h_{z,(i,v)}(\res{x}{\lcb{C}(i,v)}) \big)_{(i, v) \in I \times V}
    \end{equation}
    The pushforward model ${s(I,d,G,\pmb{v})}_*(C)$
    can therefore be expressed as a convex combination
    \begin{equation}
        x \mapsto \sum_z p_z \cdot g(\pmb{v})(x, h_z(f(\pmb{v}))(x))
    \end{equation}
    where $f(\pmb{v}), g(\pmb{v})$ are the induced maps on joint measurements and joint 
    outcomes of the simulation $s(I,d,G,\pmb{v})$.
    
    
    \begin{equation}
        x \mapsto \sum_{z} p_z \cdot \big( h_{z,i,v}(\res{x}{\lcb{C}(i)}) \big)_{(i,v) \in I \times V}
    \end{equation}
    where the value of $h_z$ on measurement site $(i,v)$
    is only a function of the measurement setting at measurement sites $\lcb{C}(i,v)$.
    
    \begin{align}
        g_i(\pmb{v})(x_i, \big( h_{z,i,v}(\res{f_i(\pmb{v})(x_i)}{\lcb{C}(i)}) \big)_{(i,v) \in \{i\} \times \supp{\pmb{v}_i}})
    \end{align}
    
    Because the circuit $C$ generates $e$ we can express $e$ as a convex combination
    of a set of functions $\{h_\lambda\}$
    where $h_\lambda(x)_{i,v} = h_{i,v,\lambda}(\res{x}{\lcb{C}(i,v)})$ for each $(i,v) \in I \times V$.
    \begin{equation}
        e(x) = \sum_\lambda p_\lambda \cdot h_\lambda(x)
    \end{equation}
    The expression of $e$ as a convex combination leads to an expression
    of $(r_n)_*(e)$ as a convex combination.
    \begin{equation}
        (s_n(\pmb{v}))_*(e_n)(x) = \sum_\lambda p_\lambda \cdot g_{\pmb{v}}(x, h_{\lambda}(f_{\pmb{v}}(x)))
    \end{equation}
    To see that $g_{\pmb{v}}(x, h_{\lambda}(f_{\pmb{v}}(x)))$
    is factorisable we restrict it to any measurement site $i \in I$.
    \begin{align}
        g_{\pmb{v}}(x, h_{\lambda}(f_{\pmb{v}}(x)))_i
        &=
        g_{i, \pmb{v}_i}(x_i, \res{h_{\lambda}(f_{\pmb{v}}(x))}{\{i\} \times \{v_{ij}\}})\\
        &= g_{i, \pmb{v}_i}(x_i, h_{\lambda,i}(\res{f_{\pmb{v}}(x)}{\bigcup_i \lcb{C}(\{i\} \times \{v_{ij}\})}))\\
        &= g_{i, \pmb{v}_i}(x_i, h_{\lambda,i}(f_{, \pmb{v}_i}(x_i)))
    \end{align}
\end{proof}

The classical bound relies upon the following lemma which we have adapted from \cite{bravyi_quantum_2018}.

\begin{definition}
    A \emph{communication graph} is a relation $R \subset A \times B$
    with the interpretation that $a \in A$ can communicate to $b \in B$
    if and only if $a \mathbin{R} b$. A communication graph on the form
    $R \subset A \times A$ is \emph{no-communication}
    if $a \mathbin{R} a' \Rightarrow a = a'$.
\end{definition}

\begin{lemma} \label{lemma:bgks-lemma}
    Let $I,V$ be finite sets and $R \subset (I \times V)^2$ a relation
    such that
    \begin{enumerate}
        \item For each $(i,v) \in I \times V$ there are at most $K$
        number of $(i',v')$ such that $(i',v') R (i,v)$.
    \end{enumerate}
    Let $u \in \dist(V \times \powset(V))$ be a distribution such that when $(v, V')$ is chosen 
    randomly according to $u$ then
    \begin{enumerate}[resume]
        \item $v$ is uniformly distributed,
        \item $V'$ has size at most $\alpha$.
    \end{enumerate}
    If $\{(v_i, V_i)\}_{i \in I}$ is chosen randomly according to the product
    distribution induced by $u$, then the probability
    that there are $i \neq i' \in I$ and $v' \in V_{i'}$
    such that $(i', v') R (i, V_i)$ is at most
    $\supp{I}^2K\alpha \supp{V}^{-1}$.
\end{lemma}
\begin{proof}
    We use a union bound over all $i \neq i' \in I$.
    For any $i \neq i' \in I$ suppose that $(v_i, V_i)$ are fixed,
    and that $(v_{i'}, V_{i'})$ are chosen randomly according to $u$.
    \begin{align}
        u(v_{i'},V_{i'} \text{ such that } (i',v_{i'}) R (\{i\} \times V_{i}))
        &\leq
        \sum_{(i', w) \in \lcb{F}(\{i\} \times V_{i})} u(v_{i'}, V_{i'} \text{ such that } v_{i'} = w)\\
        &\leq \sum_{(i', w) \in \lcb{F}(\{i\} \times V_{i})} \beta \\
        &\leq K^D \alpha \beta
    \end{align}
    The union bound therefore gives
  \begin{align}
    &u^{\prod}(\{(v_i, V_i)\}_{i \in I} \text{ such that } \exists i \neq i' \in I \text{ with } 
        (i', v_{i'}) \in \lcb{F}(\{i\} \times V_i)
        ) \\
    &\leq \sum_{i \neq i' \in I} 
        (u \times u)((v_i, V_i), (v_{i'}, V_{i'}) \text{ such that } 
            (i', v_{i'}) \in \lcb{F}(\{i\} \times V_i))\\
    &\leq \supp{I}^2 K^D \alpha \beta
  \end{align}
\end{proof}


\begin{lemma} \label{lemma:classical-bound}
    Let $C$ be a classical generating circuit of type $T(I,d,G)$
    with depth $D$ and maximal fan-in $K$.
    Let $u \in \dist(\text{Paths}(G))$ be a distribution
    on the paths in $G$
    such that when $v_1 = r, \dots, v_l$ is chosen randomly according to $u$
    we have that
    \begin{enumerate}
        \item the endpoint $v_l$ is uniformly distributed,
        \item $v_1, \dots, v_l$ is a path with endpoint $v_l$ of minimal length.
    \end{enumerate}
    Then the contextual fraction of the empirical model ${s(I,d,G, u)}_*(C)$
    simulated by $C$ through the simulation $s(I,d,G,u)$
    is at most $\supp{I}^2 K^D \supp{G}^{-1} \text{rad}(G)$.
\end{lemma}
\begin{proof}
    The pushforward model ${s(I,d,G_n,u)}_*(C)$ is by definition
    a convex combination of the pushforward models ${s(I,d,G_n,\pmb{v})}_*(C)$
    for each choice of paths $\pmb{v}$
      \begin{align} 
        {s(I,d,G,u)}_*(C) = x \mapsto \sum_{\pmb{v}} 
            u^{\prod}(\pmb{v}) \cdot {s(I,d,G,\pmb{v})}_*(C)(x) \label{eq:classical-bound-1}
      \end{align}
      The contextual fraction is the least weight
      assigned to the non-contextual part of any decomposition
      of an empirical model into a non-contextual model and another empirical
      model. From (\ref{eq:classical-bound-1}) we therefore have
      that the contextual fraction of ${s(I,d,G,u)}_*(C)$
      is bounded by the sum over all $u^{\prod}(\pmb{v})$
      such that ${s(I,d,G,\pmb{v})}_*(C)$
      is non-contextual.
    \begin{align}
        \cf{{s(I,d,G,u)}_*(C)} \leq 
            \sum_{{s(I,d,G,\pmb{v})}_*(C) \text{ is non-contextual}} u^{\prod}(\pmb{v})
    \end{align}
    By Lemma \ref{lemma:lightcones-lemma} we can weaken
    the requirement that ${s(I,d,G, \pmb{v})}_*(C)$ is non-contextual to the condition
    that there are no $i \neq i' \in I$
    with $\{v_{i1}, \dots, v_{il_i}\} \cap \lcb{C}(i, v_{il_i}) \neq \emptyset$
  \begin{align}
    \cf{{s(I,d,G,u)}_*(e)}  \leq
        \sum_{\exists i \neq i', j \leq l_{i'}
            \text{ s.t. } (i', v_{i'j}) \in \lcb{C}(i, v_{il_i}))}
                u^{\prod}(\pmb{v}) 
  \end{align}
  Finally, using Lemma \ref{lemma:bgks-lemma} with $R=\lcb{C}$
  gives that 
  \begin{align}
    \cf{{s(I,d,G,u)}_*(e)} \leq K^D \supp{I}^2 \supp{G}^{-1} \text{rad}(G)
  \end{align}
\end{proof}



\section{Generalised quantum advantage result with shallow interactive circuits} \label{section:distributing-all-measurements}

In this section we introduce a version of the distributed models
$e_{\psi,W}(G)$ given by a Weyl measurement model $e_{\psi,W}$
and a rooted graph $G$, but from any quantum realised empirical model
$e_{\psi,\pi}$. In Section \ref{section:two-round-result} we use this
to prove a quantum advantage result with shallow circuits.

To understand the intuitition for this we begin by considering the role
of the Weyl measurements in Theorem I.
To define the distributed Weyl measurement models
used in Theorem I we rely upon two tricks. First
we can perform several teleportation steps in parallel
to distribute an entangled state over long distances in a single measurement
step, up to a random Weyl operator phase at each qudit. 
Secondly, when Weyl measurements are applied to the teleported
state the correction factor $W(p)&^\dagger$ required
to retrieve the original state can be performed post measurement
as a classical operation on the outcomes.

However, observe that if the protocol is spread out over two rounds
then we can instead absorb the correction into the measurement
and apply an adaptive measurement $W(p) M W(p)^\dagger$.
The goal of this section is to use this to generalise the result
to any quantum realised empirical model.

The goal of this is to show that the fundamental thing going on about quantum
advantage is contextuality, and not restricted to Weyl measurements.
By doing this we mean to emphasise the point that at a fundamental level
the key ingredient for quantum advantage is that we can distribute
entanglement to create models that are contextual in a distributed way.

To make the idea of interacting with a circuit over several
rounds rigorous we first introduce \emph{interactive circuits}
in Section \ref{section:interactive-circuits}.
A key point here is that quantum interactive circuits and classical interactive
circuits should be considered comparable because we interact with them through
the same interface which is given by a measurement scenario.
In Section 

\subsection{Interactive circuits} \label{section:interactive-circuits}

\begin{figure}[h]
    \centering
    \begin{subfigure}{1\textwidth}
        \centering
        \includegraphics{classical-generator-two-round.pdf}
        \caption{} \label{fig:generator-two-round}
    \end{subfigure}
    \begin{subfigure}{1\textwidth}
        \centering
        \includegraphics{two-round-evaluation.pdf}
        \caption{} \label{fig:two-round-evaluation}
    \end{subfigure}
    \caption{}
\end{figure}


Although empirical models are often thought of as things that are evaluated once
it is important in for example measurement based quantum computing
that empirical models can be interacted with over several rounds.
In this section we introduce interactive circuits. They have also been used by other people.
    
\begin{definition}
Let $S = (I, \{X_i\}_{i \in I}, \{Y_{i,x}\}_{i \in I, x \in X_i})$
be a multipartite scenario. A depth $n$ interactive \emph{generating circuit}
is a deterministic classical circuit or a quantum circuit having for each $i \in I, j=1,\dots,n$:
\begin{itemize}
    \item A classical input $\text{in}_{ij}$ of type $X_i$.
    \item A classical output $\text{out}_{ij}$, such that if the input value
    to $\text{in}_{ij}$ is $x \in X_i$, then the output value of $\text{out}_{ij}$
    has type $Y_{i,x}$.
    \end{itemize}
Such that 
\begin{equation}
    \text{in}_{ij} \in \lcb{F}(\text{out}_{kl}) \implies j < l
\end{equation}
Additionally a \emph{quantum generating circuit} can use any number of qudits
prepared in the computational basis state,
and a \emph{classical generating circuit} can use any number of additional inputs
initialised according to a random seed.
\end{definition}

Interactive circuits can be thought of in two ways. Observe that the
condition on the lightcones ensures that the circuit can be evaluated in steps.
Alternatively we can think of it as a circuit
with holes where we can put in a classical circuit.

\subsection{Distributed quantum realised models} \label{section:distributed-model}
Let $e_{\psi,\pi}$ be a quantum realised empirical model
with qudits for a scenario $S = (I, \{X_i\}_{i \in I}, \{Y_{i,x}\}_{i \in I, x \in X_i})$
and $G = (V,E,r)$ a rooted graph.
We introduce an empirical model $e_{\psi,\pi}(G)$ for a scenario
$T(S,d,G)$ and a simulation from $e_{\psi,\pi}(G)$ to $e_{\psi,\pi}$
that uses two rounds.

\paragraph{Measurement scenario}
The measurement scenario $T(I,d,G)$ contains the classical information required
to perform the measurement protocol.

\begin{definition}
    Let $T(S,d,G) := (I \times V, \{X_i\}_{i \in I}, \{Y_{i,x}\}_{i \in I, x \in X_i})$
    be the multipartite scenario with measurements
    $X_i$ for each $i \in I$
    \begin{align}
        X_{i,v} := \begin{cases}
            x \mid w \mid \text{id}, &\text{if $v = r_n$}\\
            (w,x,p) \mid (w,w') \mid \text{id}, &\text{otherwise}
        \end{cases},
    \end{align}
    where $p \in \mathbb{Z}_d^2$, $\{v,w\} \neq \{v,w'\} \in E$, and outcomes
    \begin{equation}
        Y_{i,r,x} := \begin{cases}
            Y_{i,x}, &\text{if $x = p$}\\
            \mathbb{Z}_d^2, &\text{if $x = w$}
        \end{cases},
        \quad
        Y_{i,v,x} := \begin{cases}
            Y_{i,x}, &\text{if $x = (w,p)$}\\
            \mathbb{Z}_d^2, &\text{if $x = (w,w')$}
        \end{cases}
    \end{equation}
    for each $i \in I, r \neq v \in V$.
    
\end{definition}

The empirical model $e_{\psi,\pi}(G)$
is given by interpreting the measurements as follows.
The measurement settings at measurement
site $(i,r_n)$ is either
a measurement $x \in X_i$,
a neighbour $w \in V_n$ of $r_n$,
or a symbol ``id''.
Otherwise, when $v \neq r_n$, the measurement
are either a tuple $(w,x,p)$
where $w \in V_n$ is a neighbour of $v$,
$x \in X_i$, and $p \in \mathbb{Z}_d^2$,
a pair of neighbours $(w,w')$ of $v$,
or ``id''.
$e_n$ is defined as the empirical model
with quantum realisation $(\ket{\psi, G_n}, \tau_n)$
where $\tau_n$ is defined as follows.

\begin{definition}
    Let $e_{\psi,\pi}(G)$ be the quantum realised empirical model
    with state $\ket{\psi,G}$ and measurement settings
    \begin{equation}
      \tau(S,d,G,\pi) ::= (i,r) \mapsto \begin{cases}
        w \mapsto \mathcal{B}_{i, (i,r,w)}, &\\
        x \mapsto \pi(i,x)_i, &\\
        \text{id} \mapsto \text{id}_{N_G(i,r)} &
      \end{cases},
      (i,v) \mapsto \begin{cases}
        (w,w') \mapsto \mathcal{B}_{(i, v, w), (i,w,v)}, &\\
        (w, x, p) \mapsto (W(p) \pi(i,x) W(p)^\dagger)_{(i,v,w)}, &\\
        \text{id} \mapsto \text{id}_{N_G(i,v)} &
      \end{cases}
    \end{equation}
\end{definition}

\paragraph{Simulation}
Consider the following variant of the protocol
\begin{figure}[h]
  \centering
    \includegraphics{1d-teleport-final.pdf}
\end{figure}

In this figure each dot is a qudit. The first qudit
is initially in the state $\ket{\psi}$
and the remaining qudits are pairs of maximally entangled states.
Each of the pairs connected by a dotted lines are first measured in the Bell basis.
The final qudit is then measured with $W(p) M W(p)^\dagger$,
where $p = p_1 + \dots, p_{l-1}$ is the sum of the outcomes of the Bell basis measurements.



For any path $(v_1, \dots, v_l)$ in $G$
let
\begin{align}
    f_i(v_1, \dots, v_l)_1 &:= 
        (i, v) \mapsto
        \begin{cases}
          v_2, &\text{if $v=r$}\\
          (v_{j-1}, v_{j+1}), &\text{if $v=v_2, \dots, v_{l-1}$}\\
          (i,v_l) \mapsto \text{id}&
    \end{cases} \label{eq:def-a}\\
    f_i(v_1, \dots, v_l)_2 &::= (x,y_1) \mapsto \begin{cases}
      (i,v) \mapsto \text{id}, & v=v_1,\dots,v_{l-1}\\
      (i, v_l) \mapsto (v_{l-1}, x_i, \sum_{j=1}^{l-1} y_1(i, v_j)),&
    \end{cases} \label{eq:def-b}\\
    g_i(v_1,\dots,v_l) &::= (\_, \_, y) \mapsto y(i, v_l)
\end{align}

\begin{definition}
    For each choice of paths $\pmb{v} = \big( \pmb{v}_i \in \text{Paths}(G) \big)_{i \in I}$
    let $s(I,d,G,\pmb{v}):T(I,d,G) \to S(I,d)$
    be the deterministic simulation
    \begin{equation}
        s(I,d,G,\pmb{v}) :=
            ( \big(\{i\} \times \supp{\pmb{v}_i} \big)_{i \in I}, \big( f_i(\pmb{v}_i) \big)_{i \in I},
                \big(g_i(\pmb{v}_i) \big)_{i \in I}
            )
    \end{equation}
\end{definition}

\begin{definition}
    For any path distribution $u \in \dist(\text{Paths}(G))$
    let $s(I,d,G,u):T(I,d,G) \to S(I,d)$ be the probabilistic simulation
    \begin{equation}
        s(I,d,G,u) := \sum_{\pmb{v}} \prod_{i \in I} u(\pmb{v}_i) \cdot s(I,d,G,\pmb{v})
    \end{equation}
\end{definition}

\begin{lemma} \label{lemma:simulation-two-round}
    For any distribution $u \in \text{Paths}(G)$ the simulation 
    $s(S,d,G,\pi,u)$ simulates $e_{\psi,\pi}$ using $e_{\psi,\pi}(G)$ as the resource.
\end{lemma}
\begin{proof}
    After perform the 
\end{proof}

\subsection{Generating distributed quantum realised models with shallow interactive circuits} \label{section:two-round-result}
\begin{definition}
    Let $Q(S,d,G,\psi,\pi)$ be the two-round generating circuit.
    A generating circuit for $e$ is shown in Figure \ref{fig:circuit-definition-both-rounds}.
    The circuit uses a multi-qudit register initially set to the computational basis state.
    To prepare the state $\ket{\psi,G}$ the circuit
    uses a single fan-in $\supp{I}$ gate $U_\psi$,
    and a fan-in two gate $U_{i,e}$ for each $i \in I, e \in E$,
    applied in parallel.
    The state $\ket{\psi,G}$ is measured
    using a classically controlled measurement gate
    $M(i,v)$ acting on qudits $N_G(i,v)$
    and the outcome is returned.
    By definition it is easily seen that the circuit
    has depth two and maximal fan-in $\text{max}(\supp{I}, \Delta(G)+2)$.
\end{definition}

\begin{customthm}{II}
    Let $e_{\psi,\pi}$ be a quantum realised model
    in dimension $d$, $\{G_n\}_{n \in \nats}$ rooted graphs of bounded degree,
    and $\{u_n \in \dist(\text{Paths}(G_n))\}_{n \in \nats}$
    such that when $v_1, \dots, v_l$ is chosen randomly from $u_n$ then
    the endpoint $v_l$ is uniformly distributed.
    For each $n \in \nats$ write
    \begin{align}
        Q_n := Q(I,d,\psi,G_n)\\
        s_n := s(I,d,G_n,\pi, u_n)
    \end{align}
    
    The following is then true.
    $\{Q_n\}_{n \in \nats}$ is shallow and  $Q_n$ simulates $e_{\psi,\pi}$ 
    through $s_n$ for each $n \in \nats$.
    Let $\{C_n\}_{n \in \nats}$
    be a classical shallow generating circuit.
    The empirical models simulated by $\{C_n\}_{n \in \nats}$
    through $\{s_n\}_{n \in \nats}$
    have bounded contextual fraction:
    \begin{align}
            {s_n}_*(Q_n) &= e_{\psi,W}\\
        \cf{{s_n}_*(C_n)} &\in O(\supp{G_n}^{-1})
    \end{align} 
\end{customthm}
\begin{proof}
    Quantum circuits are often represented on a standard form
    consisting of a number of unitary multi-qubit gates
    followed by a computational basis measurement.
    It should be clear that the quantum circuits
    we define are equivalent to quantum circuits
    on the standard form
    with an at most $O(1)$ increase in depth and maximal fan-in.
    (2.) follows from Lemma \ref{lemma:simulation-one-round}.
    The lemmas used for (1.) and (3.) is proved in the remainder of the section.
    In Lemma \ref{lemma:quantum-circuit-lemma} we show
    that $e_n$ is generated by a quantum circuit
    of depth two and maximal fan-in $\text{max}(\supp{I}, \Delta(G_n) + 2)$.
    In Lemma \ref{lemma:classical-bound} we show that 
    $\cf{{s(I,d,G, u)}_*(e')} \leq \supp{I}^2 K^D \supp{G}^{-1} \text{rad}(G)$.
\end{proof}

\begin{example}
    For any fixed $k \in \nats$ consider Theorem I with
    $G_n := [n]^k$.
    Then $\{Q_n\}_{n \in \nats}$ is shallow.
    However, $\cf{{s_n}_*(C_n)} \in O(k^{n})$
    for any classical shallow circuit $\{C_n\}_{n \in \nats}$.
\end{example}

\begin{example}
    For any fixed $k \in \nats$
    consider Theorem I with $G_n = T_{n,k}$.
    Then $\{Q_n\}_{n \in \nats}$ is shallow (but has exponential size).
    However, $\cf{{s_n}_*(C_n)} \in O(n^{k})$
    for any classical shallow circuit $\{C_n\}_{n \in \nats}$.
\end{example}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{circuit-definition-both-rounds.pdf}
    \caption{The figure shows a simple two-round interactive quantum circuit
    that generates the empirical model $e_n$. The circuit
    first prepares a quantum register in the state
    $\ket{\psi,G_n}$, then performs two rounds of controlled measurements.
    }
    \label{fig:circuit-definition-both-rounds}
\end{figure}

\subsection{Classical bound}
The proof of the classical bound follows the same recipe as
the bound for the single-round case.
We first give a lemma that says when the reduced empirical model
is non-contextual in the deterministic case.

\begin{lemma} \label{lemma:lightcones-lemma-two}
    Let $C$ be a classical generating circuit of type $T(S,d,G)$
    and $\pmb{v} = \{(v_{i1}, \dots, v_{il_i}) \in \text{Paths}(G)\}_{i \in I}$
    a family of paths. If
    there are no $i \neq i' \in I$ with $(i,v_{il_i}) \in \lcf{C}(i', v_{i'l_{i'}})$
    then ${s(I,d,G, \pmb{v})}_*(C)$ is non-contextual.
\end{lemma}
\begin{proof}
    Because the circuit $C$ generates $e$ we can express $e$ as a convex combination
    of a set of functions $\{h_\lambda\}$
    where $h_\lambda(x)_{i,v} = h_{i,v,\lambda}(\res{x}{\lcb{C}(i,v)})$ for each $(i,v) \in I \times V$.
    \begin{equation}
        e(x) = \sum_\lambda p_\lambda \cdot h_\lambda(x)
    \end{equation}
    The expression of $e$ as a convex combination leads to an expression
    of $(r_n)_*(e)$ as a convex combination.
    \begin{equation}
        (s_n(\pmb{v}))_*(e_n)(x) = \sum_\lambda p_\lambda \cdot g_{\pmb{v}}(x, h_{\lambda}(f_{\pmb{v}}(x)))
    \end{equation}
    To see that $g_{\pmb{v}}(x, h_{\lambda}(f_{\pmb{v}}(x)))$
    is factorisable we restrict it to any measurement site $i \in I$.
    \begin{align}
        g_{\pmb{v}}(x, h_{\lambda}(f_{\pmb{v}}(x)))_i
        &=
        g_{i, \pmb{v}_i}(x_i, \res{h_{\lambda}(f_{\pmb{v}}(x))}{\{i\} \times \{v_{ij}\}})\\
        &= g_{i, \pmb{v}_i}(x_i, h_{\lambda,i}(\res{f_{\pmb{v}}(x)}{\bigcup_i \lcb{C}(\{i\} \times \{v_{ij}\})}))\\
        &= g_{i, \pmb{v}_i}(x_i, h_{\lambda,i}(f_{, \pmb{v}_i}(x_i)))
    \end{align}
\end{proof}

\begin{figure}
\centering
\begin{subfigure}{0.65\textwidth}
    \centering
    \includegraphics[scale=1.2]{c-circ-eval-tp.pdf}
    \caption{}\label{fig:c-circ-eval-tp}
\end{subfigure}
\hfill
\vrule
\hfill
\begin{subfigure}{0.3\textwidth}
    \centering
    \includegraphics[scale=1.2]{c-circ-eval-tp-simple.pdf}
    \caption{}\label{fig:c-circ-eval-tp-simple}
\end{subfigure}
\caption{}
\end{figure}


\begin{lemma} \label{lemma:classical-bound-two}
    Let $C$ be a classical generating circuit
    of type $T(S,d,G)$ of depth $D$ and maximal fan-in $K$.
    Let $u \in \dist(\text{Paths}(G))$ be a path distribution
    such that when $v_1 = r, \dots, v_l$ is chosen randomly according to $u$
    then the endpoint $v_l$ is uniformly distributed.
    The contextual fraction of the pushforward 
    ${s(I,d,G, u)}_*(C)$ is at most $\supp{I}^2 K^D \supp{G}^{-1}$.
\end{lemma}
\begin{proof}
    The proof follows the same lines as the proof of Lemma \ref{lemma:classical-bound}.
    We first write the pushforward as a convex combination
      \begin{equation}
        {s(I,d,G,u)}_*(C) = x \mapsto \sum_{\pmb{v}} 
            u^{\prod}(\pmb{v}) \cdot {s(I,d,G,\pmb{v})}_*(C)(x)
      \end{equation}
    The contextual fraction of $\cf{{s(I,d,G,u)}_*(C)}$ is therefore bounded by
    the probability that ${s(I,d,G,\pmb{v})}_*(C)$ is non-contextual.
    \begin{align}
        \cf{{s(I,d,G,u)}_*(C)} \leq 
            \sum_{{s(I,d,G,\pmb{v})}_*(e) \text{ is non-contextual}} u^{\prod}(\pmb{v})
    \end{align}
    By Lemma \ref{lemma:lightcones-lemma-two} the condition that
    ${s(I,d,G, \pmb{v})}_*(e)$ is non-contextual can be weakened
    to the condition that there are no $i \neq i' \in I$
    with $(i, v_{il_i}) \in \lcb{C}(i, v_{i'l_{i'}})$
  \begin{align}
    \cf{{s(I,d,G,u)}_*(C)}  \leq
        \sum_{\exists i \neq i'.\ (i,v_{il_i}) \in \lcb{C}(i,v_{il_i})}
            u^{\prod}(\pmb{v})
  \end{align}
  Finally, using Lemma \ref{lemma:bgks-lemma} with $R=\lcb{C}$
  gives that 
  \begin{align}
    \cf{{s(I,d,G,u)}_*(e)} \leq K^D \supp{I}^2 \supp{G}^{-1}
  \end{align}
\end{proof}
